Learning Modulo Theories

Recent techniques that integrate \emph{solver layers} into Deep Neural Networks (DNNs) have shown promise in bridging a long-standing gap between inductive learning and symbolic reasoning techniques. In this paper we present a set of techniques for integrating \emph{Satisfiability Modulo Theories} (SMT) solvers into the forward and backward passes of a deep network layer, called SMTLayer. Using this approach, one can encode rich domain knowledge into the network in the form of mathematical formulas. In the forward pass, the solver uses symbols produced by prior layers, along with these formulas, to construct inferences; in the backward pass, the solver informs updates to the network, driving it towards representations that are compatible with the solver's theory. Notably, the solver need not be differentiable. We implement \layername as a Pytorch module, and our empirical results show that it leads to models that \emph{1)} require fewer training samples than conventional models, \emph{2)} that are robust to certain types of covariate shift, and \emph{3)} that ultimately learn representations that are consistent with symbolic knowledge, and thus naturally interpretable.

==> graveyard.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% Our approach has many benefits compared to previous work such as SATNet~\cite{} and combinatorial blackbox integration into DNNs~\cite{}. Unlike SATNet, we don't require that the solver be differentiable. An advantage of this feature of our method is that we can leverage the continuous and unabated progress in solver technology being made every year. Unlike the work of Vlastelica et al.~\cite{}, our method doesn't require that the optimization objective function be linear. Perhaps most importantly, our biggest contribution is that we ground the entire space of ML systems with solver layer theoretically and show some separation results. 


% Combinatorial optimization and feature extraction are often at odds with one another and require different methods: while combinatorial optimization requires an SMT solver or symbolic logic, learning from large data requires deep learning techniques. There has been a recent trend of combining these two methods to take advantage of the benefits of each. While solvers provide explainability and allow humans to improve accuracy by incorporating logical rules, deep learning approaches can provide accuracy and can accomplish tasks rule-based learning often cannot. 

% This integration, typically of an SMT solver within a neural architecture, has varied applications. When logic is used as constraints it can allow the neural network to optimize within those constraints: for example, encoding the rules to Sudoku is done more effectively by creating logical constraints. 

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{definition}[Decomposable problem]
% \label{def:decomposable}
% Let \T be a first-order theory with constants in \Z.
% An ERM problem \D, \Hyp is \emph{decomposable} by \T if there exists a function $f: \X \to \Z$, companion hypothesis class $\Hyp_f \subseteq \X \to \Z$, and \T-formula $\phi$ such that:
% \begin{enumerate}

% 	\item For any $h \in \Hyp$, there exists $h_f \in \Hyp_f$ and $h'$ such that $h = h' \circ h_f$.

% 	\item For all $g : \Pow(\Y) \to \Y$,
% 	\begin{equation}
% 	\label{eq:decompose}
% 	L_\D(\lambda x.g(\langle x \rangle_{f,\phi})) \le \argmin_{h \in \Hyp}\, L_\D(h)
% 	\end{equation}
% 	where $\langle x\rangle_{f,\phi} = \{y : \phi(f(x), y)~\text{is satisfied}\}$.

% \end{enumerate}
% In (\ref{eq:decompose}), $f$ is called the \emph{grounding function} and $\phi$ is called the \emph{prediction logic}.
% \end{definition}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Transfer Learning}

% \begin{definition}[Representative core]
% \label{def:rep-core}
% Let \D, \Hyp be \T-decomposable by $f$ and $\phi$.
% For a measurable set $C \subseteq \X \times \Y$, define $\D\vert_C$ (similarly, $\D_f\vert_C$) to be the restriction of \D (sim. $\D_f$) to the subset of its support that intersects with $C$.
% Then $C$ is a \emph{representative core} of \D, \Hyp if and only if for any sample $S \subset \X \times \Y$, $h \in \Hyp_f$, and all $\epsilon > 0$,
% \[
% |L_{S_f \cap C}(h) - L_{\D_f\vert_C}(h)| \le \epsilon \limply |L_{S_f}(h) - L_{\D_f}| \le \epsilon
% % |L_{S_f \setminus C}(h) - L_{\D_f\vert_{\bar{C}}}(h)| \le \epsilon
% \]
% where $\bar{C} = \X \times \Y \setminus C$.
% Moreover, $C$ is minimal if none of its subsets is an $\epsilon$-representative core.
% \end{definition}

% \begin{lemma}
% Let \D be a distribution with support over \U, and $f: \U \times \V \to \mathbb{R}^{\ge0}$ be a measurable non-negative function.
% For any measurable $U \subseteq \U$, define $\D\vert_U$ to be the restriction of \D to the subset of its support that intersects $U$.
% Then for any sample $S$ taken from either \D or $\D\vert_U$ and all $v \in \V$, 
% \[
% \left|
% \Ex_{u \sim \D}[f(u, v)] - \frac{1}{|S|}\sum_{u \in S} f(u, v)
% \right|
% =
% \left|
% \Ex_{u \sim \D\vert_U}[f(u, v)] - \frac{1}{|S|}\sum_{u \in S} f(u, v)
% \right|
% \]
% \end{lemma}
% \begin{proof}
% We start by defining some additional notation to clarify the steps of the proof.
% For a subset $U \subseteq \U$ and $v \in \V$, define
% \[
% F_U(v) = \frac{1}{|U|}\sum_{u \in U} f(u, v)
% \quad\quad\quad\quad
% F_\D(v) = \Ex_{u \sim \D\vert_U}[f(u, v)]
% \]
% Note that by linearity of expectation we can decompose $F_{\D}(v) = F_{\D\vert_U}(v) + F_{\D\vert_{\bar{U}}}(v)$.
% Then by the triangle inequality,
% \[
% \begin{array}{lcl}
% 	|F_{U}(v) - F_{\D}(v)| 
% 	& \le & 
% 	|F_{U}(v) - F_{\D\vert_U}(v)| + |F_{\D\vert_U}(v) - F_{\D}(v)|
% 	\\
% 	& = &
% 	|F_{U}(v) - F_{\D\vert_U}(v)| + F_{\D\vert_{\bar{U}}}(v)
% \end{array}
% \]
% We can also reason that,
% \[
% \begin{array}{lcl}
% 	|F_{U}(v) - F_{\D\vert_U}(v)| - F_{\D\vert_{\bar{U}}}(v)
% 	& \le &
% 	|F_{U}(v) - F_{\D\vert_U}(v) - F_{\D\vert_{\bar{U}}}(v)|
% 	\\
% 	& = &
% 	|F_{U}(v) - F_{\D}(v)| 
% \end{array}
% \]
% Putting these two inequalities together, we have that $|F_{U}(v) - F_{\D}(v)| = |F_{U}(v) - F_{\D\vert_U}(v)|$.
% \end{proof}

% \begin{corollary}[Representative cores \& grounding]
% \label{corr:rep-core-ground}
% Let \D, \Hyp be \T-decomposable by $f$ and $\phi$, and $C$ be a representative core of \D.
% Then for non-negative loss $\ell$, any $S \sim \D$ that is $\epsilon$-sufficient for grounding on \D, \Hyp is also $\epsilon$-sufficient for grounding on $\D\vert_C$, \Hyp, and vice versa.
% \end{corollary}

% \begin{theorem}[Grounding samples transfer by core]
% Let \D, \Hyp be \T-decomposable by $f$ and $\phi$, and $S \sim \D$ be $\epsilon$-sufficient for grounding with respect to a bounded loss $\ell$.
% Then for any $\D'$ that shares a minimal representative core $C$ with \D and any $h \in \Hyp_f$,
% \[
% 	|L_{S_f}(h) - L_{\D'_f}(h)| \le \epsilon + \|\ell\|_\infty\TV(\D_f\vert_C, \D'_f\vert_C)
% \]
% Above, \TV is the total variation distance, which is defined as $\TV(\D, \D') := \sup_S |\D(S) - \D'(S)|$.
% \begin{proof}
% We have that $|L_{S_f \cap C}(h) - L_{\D_f\vert_C}(h)| \le \epsilon$, by Corollary~\ref{corr:rep-core-ground} and the fact that $S$ is $\epsilon$-sufficient for grounding.
% \emph{To be continued...}
% \end{proof}

% \end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% \paragraph{Case 2: $\mathsf{sign}(y) \ne \mathsf{sign}(\hat{y})$.}
% In this case, the two algorithms behave differently.
% We start by analyzing $\backcore^\phi$.
% Because of assumption (2), the minimal unsatisfiable core computed at line 9 will consist of a single clause $z_i = z_b[i]$ for some index that does not match the (unique) correct value of $z^\star$ satisfying $\phi(z^\star, \hat{y})$, and moreover that $z^\star[i] = 1 - \mathrm{sign}(z[i])$.
% Then the vector returned by $\backcore^\phi$ will be:
% \begin{equation}
% \left(
% 0, \ldots, \partial_{z[i]} \ell(z[i], z^\star[i]), \ldots, 0
% \right)
% \end{equation}
% This is a subgradient of $\ell(h_f(\cdot), z^\star)$ at $z$, as for any $z'$, 
% \[
% \begin{array}{ll}
% &
% \ell(z, z^\star) + 
% \langle z' - z, (0, \ldots, \partial_{z[i]} \ell(z[i], 1 - \mathsf{sign}(z[i])), \ldots, 0)\rangle
% \\
% = &
% \ell(z, z^\star) + (z'[i] - z[i]) \cdot \partial_{z[i]} \ell(z[i], 1 - \mathsf{sign}(z[i]))
% \end{array}
% \]

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{theorem}
% Let \D, \Hyp be a \T-decomposable problem with grounding function $f$ and prediction logic $\phi$ where:
% \begin{enumerate}
%     \item \Z and \Y are cartesian products of the Boolean domain.
%     \item For any $(x, y) \sim \D$ and $y' \ne y$, $\phi(f(x), y')$ is \T-equivalent to false.
%     \item The loss $\ell^\phi = \lambda z. \lambda y^\star. \ell(\backcore^\phi(z, \forward^\phi(z), \partial_y\ell(y, y^\star)), y^\star)$ is convex in $z$ for any fixed $y^\star$.
% \end{enumerate}
% Then given $z, y$, $\partial_y \ell(y, y^\star)$, and $\phi$, where $(\cdot, y^\star) \sim \D$, $z \in \mathbb{R}^p$, and $y = \forward(z, \phi)$, the output of Algorithm~\ref{alg:core-backprop}, $\backcore(z, y, \partial_y\ell(y, y^\star))$, is a subgradient of the loss $\ell^\phi$.
% \end{theorem}

% \begin{proof}
% Recall that for a convex function $f$, a subgradient of $f$ at $x_0$ is a vector $v$ such that for any $x$, $f(x) \ge f(x_0) + \langle x - x_0, v \rangle$.
% So we must show that for a given set of inputs $z$ and $y$ and output $\dot{z}$ of Algorithm~\ref{alg:core-backprop}, Equation~\ref{eq:subgrad-goal} is true.
% \begin{equation}
% \label{eq:subgrad-goal}
%     \forall z'. \ell^\phi(z', y^\star) \ge \ell^\phi(z, y^\star) + \langle z' - z, \dot{z}\rangle 
% \end{equation}
% First observe that the sign of $\hat{y}$ computed on line 3 must be equal to that of $y^\star$.
% This follows from two facts:
% \begin{enumerate} 
%     \item At any coordinate $i$ where $y[i] \ne y^\star[i]$, $\mathsf{sign}(\partial_y\ell(y, y^\star))[i] = \mathsf{sign}(y)[i]$.
%     \item At any coordinate $i$ where $y[i] = y^\star[i]$, $\mathsf{sign}(\partial_y\ell(y, y^\star))[i] = -1 \cdot \mathsf{sign}(y)[i]$.
% \end{enumerate}
% Having established the correctness of $\hat{y}$, observe that $\forward^\phi$ is piecewise differentiable everywhere except where at least one coordinate of $z$ is $0$, with
% \[
% \frac{\partial}{\partial z} \forward^\phi(z) = 
% \left\{
% \begin{array}{ll}
% 0 & \forall 0 \le i < p. z[i] \ne 0 \\
% \mathrm{undefined} & \mathit{otherwise}
% \end{array}
% \right.
% \]

% Now there are two cases to consider.
% \paragraph{Case 1: $\mathsf{sign}(y) = \mathsf{sign}(\hat{y})$.}
% In this case $\dot{z} = \partial_z \ell(z, \mathsf{sign}(z))$. 
% Note that if $\ell^\phi(\cdot, \hat{y})$ is differentiable at $z$, then $\dot{z} = \partial_z \ell(z, \mathsf{sign}(z)) = \partial_z \ell^\phi(z, y^\star)$, so the result is a subgradient.
% Otherwise,

% \paragraph{Case 1: $\mathsf{sign}(y) \ne \mathsf{sign}(\hat{y})$.}


% \end{proof}

==> section_discuss.tex <==

\section{Discussion \& Limitations}

==> section_learning_theories.tex <==
%!TEX root=./main.tex

\section{Learning with Theories}
\label{sect:theory}

In this section, we examine a class of learning problems in which a first-order theory solver is used alongside ERM.
Our focus is on inference tasks that require two distinct types of reasoning to succeed: translating data into meaningful high-level symbols, i.e. perception or \emph{grounding}, and prediction over these symbols by a formalized set of principles.
We model settings where grounding is carried out by a function learned via ERM, and prediction is handled by a theory solver that is given a formula $\phi$ and a set of inputs from the perception function.
We call this learning framework \ermphi, and aim to characterize several of its properties.

Section~\ref{sect:theory-basics} provides the definition of \ermphi and a class of \emph{decomposable} learning problems that are amenable to this setting, several examples of problems that we will use throughout the paper. 
Decomposable problems are comprised of data whose labels are generated by the composition of a \emph{grounding function} and the first-order prediction logic $\phi$.
A general strategy for solving these problems is to generate a \emph{grounding sample} from $\phi$ (Definition~\ref{def:ground-sample}), 
and apply traditional ERM on it to approximate the grounding function.
However, Theorem~\ref{thm:hard-grounding} shows that doing so is computationally hard, giving a lower bound on its worst-case complexity---regardless of the complexity of solving $\phi$.
Section~\ref{sect:theory-solving} then examines how $\phi$ contributes to the learnability of a decomposable problem via \ermphi.
Theorem~\ref{lemma:bijective-learnable} identifies conditions for which the solution is straightforward and efficiently solvable, and Theorem~\ref{thm:groundable} generalizes this result to problems whose solutions might not be found efficiently, but are learnable in \ermphi nonetheless.


\subsection{Decomposable Learning Problems}
\label{sect:theory-basics}

We begin by formalizing the class of learning problems that will remain the central focus throughout the paper.
Definition~\ref{def:groundable} states the requirements for a \emph{decomposable learning problem}.

\begin{definition}[Decomposable problem]
\label{def:decomposable}
Let \T be a first-order theory with constants in \Z.
An ERM problem \D, \Hyp is \emph{decomposable} by \T if there exists a function $f: \X \to \Z$, companion hypothesis class $\Hyp_f \subseteq \X \to \Z$, and \T-formula $\phi$ such that:
\begin{enumerate}

	\item For any $h \in \Hyp$, there exists $h_f \in \Hyp_f$ and $h'$ such that $h = h' \circ h_f$.

	\item There exists a random function $g : \Pow(\Y) \to \Y$ such that for any $n > 0$,
	\[
	\label{eq:decompose}
	\forall S \in \supp\,\D^n. 
		\Pr_{(x, y) \sim \D}[(x, y) \in S] = \Pr_{(x, \cdot) \sim \D}[(x, g(\langle x \rangle_{f,\phi})) \in S]
	\]
	where $\langle x\rangle_{f,\phi} = \{y : \phi(f(x), y)~\text{is satisfied}\}$.
\end{enumerate}
In (\ref{eq:decompose}), $f$ is called the \emph{grounding function} and $\phi$ is called the \emph{prediction logic}.
\end{definition}

Intuitively, a learning problem defined in terms of a distribution \D and hypothesis class \Hyp is decomposable if members of \Hyp can be decomposed into functions that are responsible for grounding and prediction, and \D can be expressed in terms of a grounding function and a first-order predictive theory $\phi$.
There are a few important things to note.
First, there is no requirement that the grounding function $f$ be a member of $\Hyp_f$.
While this may be realized at times, we should not assume that the data is actually generated, or otherwise described with perfect fidelity, by a function in the class that one learns over.
In fact, we do not assume that $f$ is efficiently computable, as it may correspond to a process in nature, or an aspect of data generation that is not understood well enough to make such computational claims.

Second, for a given $x$, there may be more than one satisfying assignment for $y$ to $\phi(f(x), y)$.
The function $g$ in (2) accounts for this, requiring only that when solutions to $\phi(f(x), y)$ are sampled by $g$, the result is distributed identically to \D.
This paper will focus on the case where satisfying assignments for $y$ are unique, as these are more in line with ERM classification problems.
We leave exploration of the more general setting to future work.

Before illustrating several examples of decomposable problems, we note that if the grounding function is known, can be computed efficiently, and $\phi$ is efficiently solvable, then the learning problem effectively has a closed-form solution.
Rather, we assume that only $\phi$ and perhaps $g$ are known, and a sample of \D is given.
The remaining challenge is to identify a grounding hypothesis $h_f \in \Hyp_f$ for which the construction in (2) is an effective solution to the end-to-end learning problem posed by \D, \Hyp.
This stands in contrast to traditional ERM, in which a good solution $h \in \Hyp$ must either solve both grounding and prediction, or find a ``shortcut'' that manages to predict \D as well as the decomposition.

\begin{figure*}[t]
\begin{center}
\begin{tikzpicture}[
label/.style 2 args={
  postaction={
    decorate,
    transform shape,
    decoration={
      pre length=1pt, post length=1pt,
      markings,
      mark=at position #1 with \node #2;
      }
  }
}  
]

\node[inner sep=0pt] (features) at (-0.5,1.5) 
	{Features \X};
\node[inner sep=0pt] (four) at (-0.5,0)
    {\includegraphics[width=.1\textwidth]{figures/mnist4.png}};
\node[inner sep=0pt] (seven) at (-0.5,-2)
    {\includegraphics[width=.1\textwidth]{figures/mnist7.png}};
\draw[thick] ($(four.north west)$) rectangle ($(seven.south east)$);

\node[inner sep=0pt,text width=3cm,align=center] (zdomain) at (4,1.5) 
	{Symbolic Domain \Z};
\node[inner sep=5pt] (bv_rep) at (4,1) 
{$\mathsf{0010000111}$};


\draw[->,thick,bend right] ($(four.north east)!0.5!(seven.south east)$) 
							to [out=320,in=150] 
							node [pos=0.55,yshift=-4ex,xshift=4ex,align=center,text width=3cm] 
								{\small Grounding \\ Function $f$}
							(bv_rep.west);

\node[inner sep=1pt] (logic) at (7.5,-1.5) 
	{
	$\arraycolsep=1pt
	\begin{array}{ll}
		\phi(\quad z_1\|\ldots\|z_{10}, \quad y \quad)\ \equiv & \\
		a = \indicator_{z_1 > 0}\| \ldots \| \indicator_{z_5 > 0} \land 
		b = \indicator_{z_5 > 0} \| \ldots \| \indicator_{z_{10} > 0} & \land \\
		a + b = y &
	\end{array}
	$};
\node[inner sep=5pt,text width=3cm,align=center,below of=logic,yshift=-1ex] (f) {Prediction Logic $\phi$};

\node[inner sep=0pt,text width=3cm,align=center] (f) at (7.5,1.5) 
	{Labels \Y};
\node[inner sep=5pt] (result) at (7.5,1) 
	{$\{\mathsf{01011}\}$};

\draw[->,thick] (bv_rep.south) to [out=270,in=90] ([xshift=-13ex]logic.north);
\draw[->,thick] ([xshift=-3.5ex]logic.north) to [out=100,in=270] 
				node [pos=0.5,xshift=7ex,align=center,text width=3cm] {\small Satisfying \\ Assignments} 
				(result.south);
\end{tikzpicture}
\end{center}
\caption{\label{fig:mnist-example} MNIST Addition example (Example~\ref{ex:mnist-add}).}
\end{figure*}

\subsubsection{Examples}

While it is conceivable that nearly any problem suitable for ERM could be cast in terms of Definition~\ref{def:decomposable}, it may not always be useful or feasible to do so.
For example, one could use a trivial $\phi$ that simply equates $f(x)$ and $y$, in which case the decomposition says nothing about the structure of the learning problem or its solutions.
Alternatively, one might suppose that a perception problem, such as handwritten symbol or speech recognition, can be decomposed by a well-crafted $\phi$ in \emph{some} theory and a corresponding $f$.
Our focus is not on these hypothetical cases, but instead on problems for which domain knowledge presents a well-defined logical theory, which can be leveraged with existing solvers assuming a solution to the perception problem.
To further illustrate this, we present a few simple examples of such problems.
Additional examples are covered in Section~\ref{sect:eval}.

\begin{example}[MNIST Addition]
\label{ex:mnist-add}
A canonical example of a decomposable problem is MNIST Addition.
Samples consist of an image containing to $28 \times 28$ grayscale images of handwritten digits, and labels are the sum of the digits depicted in each image.
Formally, $\X = \mathbb{R}^{56 \times 28}$, and $\Y = \{0,1\}^5$ represents bitvectors of length 5, i.e., the minimal length needed to encode the sum of pairs of single digits.
The support of \D is the subset of \X containing pairs of MNIST digits.
The grounding function $f : \X \to \mathbb{R}^{10}$ takes images of paired digits, and produces a real vector of size 10 that the prediction logic $\phi$ interprets as two bitvectors of length 5:
\begin{equation}
\label{eq:add-theory}
		\phi(z_1\|\ldots\|z_{10}, y) \equiv 
		a = \concat(\indicator_{z_1 > 0}, \ldots, \indicator_{z_5 > 0}) \land 
		b = \concat(\indicator_{z_5 > 0}, \ldots, \indicator_{z_{10} > 0}) \land
		a + b = y 
\end{equation}
The prediction logic is the formula $\phi(z_1, z_2, y) := y = z_1 + z_2$, in the combined theory of real arithmetic and arithmetic over bitvectors of length 5.

Supposing that the hypothesis space \Hyp is depth-$d$ feedforward neural networks, where $d = d_1 + d_2$ and the representation at layer $d_1$ is in $\mathbb{R}^{10}$, then $\Hyp_f$ would consist of depth-$d_1$ networks representing functions $\X \to \mathbb{R}^{10}$ that take images to pairs of length 5 bitvectors.

The artificial nature of this example as a learning problem is noted.
Labels for MNIST digits are readily available, so a natural way to solve this problem is to train a supervised model that predicts the corresponding bitvector label for an instance, and simply combine the resulting model with an SMT solver (or a simpler routine that can perform addition).
However, we will use this example throughout the paper to illustrate key ideas in a simple, clear setting, as a proxy for more complex decomposable problems for which such intermediate labels are not available, or would be expensive to obtain.
Additionally, MNIST addition has been used as a common benchmark in prior work on neuro-symbolic learning~\cite{huang2021scallop,manhaeve2018deepproblog,bloice19mnistaddition,kim21symbregression}, so it is likely familiar to many readers.
\end{example}

\begin{example}[Visual Algebra]
\label{ex:visual-alg}
A somewhat more involved variant of Example~\ref{ex:mnist-add} takes handwritten images of algebra problems of the form $ax + b = c$.
To keep things concrete without introducing unnecessary complexity, assume that $a, b$ and $x$ are a single positive digit (i.e., $0 < a, b, x \le 9$), so that $0 < c \le 90$ and $\Y = \{0,1\}^4$.

As in Example~\ref{ex:mnist-add}, suppose that the hypothesis space \Hyp is depth-$d$ feedforward neural networks, where $d = d_1 + d_2$. 
There are several forms that the latent space \Z can take, but it must encode the values for $a, b$, and $c$ shown in each instance $x \in \X$.
We assume that it encodes $a$ and $b$ as 4-bit bitvectors, and $c$ as two 4-bit bitvectors $c_1, c_2$ such that $c = 10*c_1 + c_2$.
This leaves open hypotheses that use the same weights to recognize all of the relevant digits in an instance, rather than learning several redundant sets of weights for digits at different positions.

Then the representation at layer $d_1$ is in $\mathbb{R}^{16}$, and $\Hyp_f$ consists of depth-$d_1$ networks representing functions $\X \to \mathbb{R}^{16}$.
\D, \Hyp is decomposable by a grounding function that extracts the four relevant bitvectors from each $x \in \X$, and $\phi$ (Equation~\ref{eq:arith-theory}) is in the combined theory of real and bitvector arithmetic.
\begin{equation}
\label{eq:arith-theory}
	\begin{array}{lcll}
		\phi(z_1\|\ldots\|z_{16}, y) & \equiv &
		a = \concat(\indicator_{z_1 > 0}, \ldots, \indicator_{z_4 > 0}) \land
		b = \concat(\indicator_{z_5 > 0}, \ldots, \indicator_{z_8 > 0}) & \land \\
		& &
		c_1 = \concat(\indicator_{z_9 > 0}, \ldots, \indicator_{z_{12} > 0}) \land
		c_2 = \concat(\indicator_{z_{13} > 0}, \ldots, \indicator_{z_{16} > 0}) & \land \\
		& &
		c = 10c_1 + c_2 \land ay + b = c 
	\end{array}
\end{equation}
Note that the conditions in Definition~\ref{def:decomposable} are satisfied.
The first follows from the architecture described above.
For the second, observe that for any $z$, $\phi(z, y)$ has one satisfying assignment for $y$, so any random function $g : \Pow(\Y) \to \Y$ will suffice.
Then for any instance $x, y$ and the correct bitvector representation of the digits $f(x)$, $g(\langle x\rangle_{f,\phi}) = y$.
\end{example}

\subsection{\ermphi Learning and Sample Sufficiency}
\label{sect:theory-sufficiency}

Given a grounding function $f$ and distribution $\D_\X$ over \X, let $\D_{f(\X)}$ be the image of $\D_\X$ under $f$.
One way to solve a decomposable problem \D, \Hyp, assuming the prediction logic is known, is to reduce it to an easier supervised ERM problem.
Namely, if the ERM problem $\D_\X \times \D_{f(\X)}$ for some hypothesis class $\Hyp'$ is more easily learnable than the original, then it is advantageous to look for ways to solve it.
Doing so requires a \emph{grounding sample} (Definition~\ref{def:ground-sample}) over which to minimize risk.

\begin{definition}[Grounding sample]
\label{def:ground-sample}
Let \D, \Hyp be a \T-decomposable problem with grounding function $f$.
The grounding sample $S_f$ for $S \sim \D$ is given by
$[(x_i, f(x_i)) : (x_i, y_i) \in S]$, i.e., tuples that consist of the first element of each instance in $S$ and its image under $f$.
\end{definition}

If a sufficient grounding sample can be obtained, then the construction shown in (\ref{eq:decompose}) yields a model that will predict samples from \D, by applying ERM to learn a suitable approximation of $f$~\footnote{Note that this may be an improper solution to the original problem, because (\ref{eq:decompose}) may not be in \Hyp; for practical purposes, we assume that this is not a concern as long as solving $\phi$ can be done efficiently in practice.}.
This is the central idea of \ermphi, stated in Definition~\ref{def:ermphi}.

\begin{definition}[\ermphi learning principle]
\label{def:ermphi}
Let \D, \Hyp be a \T-decomposable problem with grounding function $f$, prediction logic $\phi$, and $g$ satisfying Definition~\ref{def:decomposable}.
Then the \ermphi solution $\hat{h}$ to \D, \Hyp composes a solver for $\phi$ with the empirical minimizer $\hat{h_f}$ of the grounding sample $S_f$:
\[ 
\hat{h}_f = \argmin_{h_f \in \Hyp_f} L_{S_f}(h_f),\quad\quad \hat{h} = \lambda x.g(\langle x \rangle_{h_f},\phi),
\]
If $\hat{h}_f$ is not unique, then neither is the \ermphi solution.
\end{definition}

Our goal is to characterize settings where the \ermphi solution generalizes well, i.e., its empirical risk on the training sample is not far from its true risk on \D, and ideally, generalizes at least as well as the ERM solution.
To develop this result, we adapt the notion of an $\epsilon$-sufficient training sample from ERM (Definition~\ref{def:eps-sufficient}) to our setting.
We will build on a fundamental result that $\epsilon$-sufficiency gives an upper bound on loss for any model produced by ERM (Lemma~\ref{lemma:erm-sufficient-bound}).

\begin{definition}[$\epsilon$-sufficient sample]
\label{def:eps-sufficient}
A sample $S \sim \D$ is $\epsilon$-sufficient for \D, \Hyp and loss function $\ell$ if and only if
$
	\forall h \in \Hyp. |L_S(h) - L_\D(h)| \le \epsilon
$.
\end{definition}
\begin{lemma}[{\citeauthor[Chapter~3]{shalev-shwartz-2014}}]
\label{lemma:erm-sufficient-bound}
Let $S \sim \D$ be an $\nicefrac{\epsilon}{2}$-sufficient sample for hypothesis class \Hyp and loss $\ell$. 
Then for any $h = \argmin_{h \in \Hyp}(L_S(h))$, it follows that $L_S(h) \le L_\D(h) + \epsilon$.
\end{lemma}

The variant of $\epsilon$-sufficiency shown in Definition~\ref{def:eps-sufficient-ground} identifies samples that have this potential.
We note that samples that satisfy Definition~\ref{def:eps-sufficient-ground} may not lead to a solution for the corresponding \ermphi problem, as it does not guarantee that the grounding sample can be generated or approximated.
We will address this question further in Section~\ref{sect:theory-solving}.

\begin{definition}[$\epsilon$-sufficient for grounding]
\label{def:eps-sufficient-ground}
Let \D, \Hyp be a \T-decomposable problem with grounding function $f$, and $\Hyp_f$ be defined as in Definition~\ref{def:decomposable}.
A sample $S \sim \D$ with corresponding grounding sample $S_f$ is $\epsilon$-sufficient for grounding if and only if: 
$
	\forall h \in \Hyp_f. |L_{S_f}(h) - L_{\D_f}(h)| \le \epsilon
$.
\end{definition}

A sample may be sufficient for grounding, but not $\epsilon$-sufficient in the sense of Definition~\ref{def:eps-sufficient}.
Intuitively, the sample may contain enough information to specify a grounding function that generalizes, but leave $\phi$ underspecified.
This is illustrated in Example~\ref{ex:grounding-addition-algebra}.
We believe that this demonstrates a key advantage of solving \ermphi rather than the traditional ERM problem.

\begin{example}[Sufficient samples for MNIST Addition]
\label{ex:grounding-addition-algebra}
Recall the MNIST addition problem from Example~\ref{ex:mnist-add}.
Recall that $\X = \mathbb{R}^{56 \times 28}$, and let $\Hyp_g \subseteq \X \to \mathbb{R}^5$.
Then consider the class of functions shown in Equation~\ref{eq:ex-grounding-addition}.
\begin{equation}
\label{eq:ex-grounding-addition}
\Hyp_f = \left\{
	h :
	\exists g \in \Hyp_g. h(x) = g(x\mathtt{[{:}28]}) \| g(x\mathtt{[28{:}]})
\right\}
\end{equation}
In words, the functions in the companion hypothesis class $\Hyp_f$ are defined in terms of a function in $\Hyp_g$ that is applied first to the left digit, then to the right digit, and the results are concatenated.
Then for any \Hyp that adopts this compantion hypothesis class, samples that consist only of repetitions of the same digit may be sufficient for grounding.

In more detail, let $S \subset \mathbb{R}^{28 \times 28}$ be a finite, $\sqrt{\epsilon}$-sufficient sample for the ERM problem of MNIST classification over hypothesis class $\Hyp_g$.
Then $S_+ = [(x, x) : x \in S]$ is $\epsilon$-sufficient for grounding over $\Hyp_f$.
To see why, observe that for any $g \in \Hyp_g$, $L_S(g) = L_{S_+}(\lambda x. g(x\mathtt{[{:}28]})\|g(x\mathtt{[28{:}]}))$.
Then for $g^\star = \argmin_{g \in \Hyp_g} L_S(g)$, assuming 0-1 loss it must be that:
\begin{align*}
	h^\star = \argmin_{h \in \Hyp_f} L_{S_+}(h) &=
	\argmin_{h = \lambda x. g(x\mathtt{[{:}28]})\|g(x\mathtt{[28{:}]})} \min_{g \in \Hyp_g} L_{S_+}(h) 
\\ &=
	\argmin_{h = \lambda x. g(x\mathtt{[{:}28]})\|g(x\mathtt{[28{:}]})} \min_{g \in \Hyp_g} L_S (g)
\\ &=
	\lambda x . g^\star(x\mathtt{[{:}28]})\|g^\star(x\mathtt{[28{:}]})
\end{align*}
Assuming that instances in the MNIST addition distribution $\D_+$ sample pairs from MNIST digits independently, the error rate of $h^\star$ on $\D_+$ is the square of $g^\star$'s error rate on the distribution of MNIST digits $\D$.
Then it follows that $S_+$ is $\epsilon$-sufficient for grounding on $\D_+$.
$\square$
\end{example}

Before moving on to our analysis of solvable \ermphi instances, we conclude this section with a result on the feasibility of generating grounding samples in general settings.
Theorem~\ref{thm:hard-grounding} shows that even when the prediction logic is efficiently decidable, generating a grounding sample may be hard.
The reason for this is that we do not place any computational restrictions on the grounding function $f$. 
It is a component of the data distribution, which may correspond to natural processes that are not efficiently computable.
It may be the case that if the complexity of $f$ is bounded, then upper bounds can be placed on the complexity of generating a grounding sample.
We leave this exploration for future work.

\begin{theorem}[Grounding samples are hard to generate]
\label{thm:hard-grounding}
Let \D, \Hyp be decomposable by theory \T for grounding function $f$ and prediction logic $\phi(z, y)$.
Regardless of the complexity of deciding \T, given $S \sim \D$, generating the grounding sample $S_f$ is NP-Hard.
\end{theorem}
\begin{proof}
We show a reduction from propositional satisfiability to the problem of identifying the grounding sample for $S$ taken from a particular distribution.
Given a CNF formula $P$, we show how to construct a distribution \D whose grounding sample maps to \emph{unsat} if $P$ is unsatisfiable, and a satisfying assignment otherwise.
The grounding function $f$ plays the most important role in this reduction, and we exploit the fact that $f$ need not be efficiently computable.
Note that $f$ does not need to be evaluated to perform the reduction, so this does not affect the complexity of the reduction itself.

The features of \D encode propositional formulas in CNF with three literals per clause, over $n$ variables, and $m$ clauses.
Then $\X = \{-1, 0, 1\}^{m \times n}$, where $x_{ij} = -1$ gives that the $j$th variable in the $i$th clause is negated, $x_{ij} = 0$ that the $j$th variable is not present in the $i$th clause, and otherwise that the $j$th variable is positive.
Then for a given CNF $P$, define $f: \X \to \{-1,1\}^n$ to return a satisfying assignment to $P$ if one exists, and $\mathbf{0}$ otherwise.
\[
f(x) =
\left\{
\begin{array}{ll}
	z~\text{s.t.}~m = \sum_{0<i\le m}\,\max_{0<j\le n}\,x_{ij} z_j & P~\text{is satisfiable} \\
	\mathbf{0} & \text{otherwise}
\end{array}
\right.
\]

The prediction logic used to generate \D with $f$ plays a smaller role, but it cannot be entirely forgotten about.
Some trivial choices, e.g., $\phi(z, y) := y = z$, that map the output $z$ of $f(x)$ directly to $y$ (and related variants) do not work because it is straightforward to recover the grounding sample given $(x, y) \sim \D$.
Any bijective formula does not fit the needs of the theorem statement, as Lemma~\ref{lemma:bijective-learnable} illustrates that in these cases the grounding sample could be computed in $|S| \times \mathrm{poly}(|z|)$.
So solutions for $z$ to $\phi(z, y)$ given $y$ must be surjective.
The trivially-satisfiable formula $\phi(z, y) := y = 0$ suits our needs.

Putting these elements together, define \D over $\{-1, 0, 1\}^{m \times n} \times \{0\}$ with support over the singleton set $(P^\text{enc}, 0)$, for the encoding $P^\text{enc}$ of $P$ into $\{-1, 0, 1\}^{m \times n}$.
The only non-empty sample $S$ of \D is this tuple, and its grounding sample $S_f$ is $(P^\text{enc}, z^\text{sat})$.
Note that $z^\text{sat} = \mathbf{0}$ if and only if $P$ is unsatisfiable.
The binary representation of $P^\text{enc}$, $\phi$, and $S$ can be constructed in $\mathrm{poly}(m \times n)$, the size of $P$.
Given an algorithm $G$ that takes this representation and returns the grounding sample, which is also polynomial in $m \times n$, one can determine whether $P$ is satisfiable by comparing the result with $\mathbf{0}$.
\end{proof}

\subsection{Solvable instances of \ermphi}
\label{sect:theory-solving}

We turn to answering the following question: when does the sufficiency of a training sample ensure that the \ermphi solution will perform well?
While the connection between sample sufficiency and generalization is clear in traditional ERM, this is not the case for \ermphi.
Theorem~\ref{thm:hard-grounding} shows that it may not be feasible to generate a grounding sample for computational reasons, but irrespective of the cost, it may be that there is not enough information to be gained from $\phi$ and a sample of \D to solve \ermphi.

In this section, we identify conditions on $\phi$ which imply that the \ermphi solution is approximately optimal given a sample that is sufficient for grounding.
Theorem~\ref{lemma:bijective-learnable} identifies conditions under which this is possible by making a linear number of queries to a \T-solver in the size of the training sample.
It does not address the complexity of the remaining ERM problem, but by limiting the additional complexity of the \ermphi problem, it characterizes a setting where successful learning can occur given only a grounding-sufficient sample, and the cost is likely to be dominated by traditional ERM.
On the other hand, Theorem~\ref{thm:groundable} imposes fewer conditions on $\phi$, and is likely applicable to more realistic decomposable problems.
But it does not bound the number of queries needed to the solver, and the construction used in its proof would not yield a feasible solution in practice.

\begin{theorem}
\label{lemma:bijective-learnable}
Let \D, \Hyp be decomposable by a decidable theory $T$ for grounding function $f$ and prediction logic $\phi(z, y)$.
If the following conditions hold:
\begin{enumerate}
    \item For any $(x, y) \sim \D$ and $y' \ne y$, $\phi(f(x), y')$ is \T-equivalent to false and there is exactly one $z$ such that $\phi(z, y)$ is \T-equivalent to true.
	\item $S$ is $\nicefrac{\epsilon}{2}$-sufficient for grounding over $\Hyp_f$ with respect to the 0-1 loss $\ell^{01}$.
\end{enumerate}
Then the \ermphi solution $\hat{h}$ yields:
\[
	L^{01}_\D(\hat{h}) \le \min_{h \in \Hyp}\, L^{01}_\D(h) + \epsilon
\]
Moreover, finding this solution requires at most $|S|$ queries to a \T-solver.
\end{theorem}
\begin{proof}
We must show that the we can use ERM to approximate $f$, and that the construction from Equation~\ref{eq:decompose} satisfies the claimed generalization bound.
$T$ is decidable, so we can generate the grounding sample $S_f$ for $S$ by solving for $z$ in $\phi(z, y)$ for each $(x, y)$ in $S$.
That this is the grounding sample follows from the asumpation that for $(x, y) \sim \D$ and $y' \ne y$, $\phi(f(x), y')$ is false, and that there is exactly one $z$ such that $\phi(z, y)$ is true.
Thus, for any $x, y$ in the support of \D, if $z$ satisfies $\phi(z, y)$, then it follows that $z = f(x)$.

Let $h^\star = \argmin_{h \in \Hyp}\, L_\D(h)$.
Definition~\ref{def:decomposable} has that $h^\star = h'^\star \circ h^\star_f$ for some $h'^\star$ and $h^\star_f \in \Hyp_f$.
We will show that $h^\star_f$ can be approximated using ERM on $S_f$.
Let $h_{S_f}$ be any result obtained by ERM learning on $S_f$ over $\Hyp_f$, and $\D_f$ be the distribution of grounding samples for \D.
In other words,
\[
\Pr_{(x, f(x)) \sim \D_f}[(x, f(x))] 
	= \int\limits_{y : (x, y) \in \supp(\D)} \Pr_{(x,y) \sim \D}[(x,y)]\,dy
\]
Observe that $S_f$ is distributed by $\D_f^n$, if $n = |S_f|$.
$S$ is $\nicefrac{\epsilon}{2}$ sufficient for grounding over $\Hyp_f$ with respect to $L^{01}$, so 
for all $h \in \Hyp_f$, 
\[
\begin{array}{ccccc}
	L^{01}_{\D_f}(h_{S_f}) 
	&\le L^{01}_{S_f}(h_{S_f}) + \nicefrac{\epsilon}{2} 
	&\le L^{01}_{S_f}(h) + \nicefrac{\epsilon}{2} 
	&\le L^{01}_{\D_f}(h) + \nicefrac{2\epsilon}{2}
	&= L^{01}_{\D_f}(h) + \epsilon
\end{array}
\]
This includes $h^\star_f$, which means that the error rate of $h_{S_f}$ on grounding is near that of the empirical risk minimizer $h^\star_f$.
Then consider the function $\hat{h} = \lambda x.g(\langle x \rangle_{h_{S_f}, \phi})$, where $g$ is any function from $\Pow(\Y)$ to \Y.
By condition (1), $\langle x \rangle_{h_{S_f}, \phi}$ will be singleton, so $\hat{h}$ will always return the correct $y$ whenever $f(x) = h_{S_f}(x)$. 
From this, one has:
\[
\begin{array}{ll}
	L^{01}_\D(\hat{h})
	&= \Pr_{(x, y) \in \D}[h_{S_f}(x) \ne f(x)] \\
	&= \Pr_{(x, z) \in \D_f}[h_{S_f}(x) \ne z] \\
	&\le L^{01}_{\D_f}(h^\star_f) + \epsilon \\
	&\le L^{01}_\D(h^\star) + \epsilon
\end{array}
\]
The last inequality follows from condition (1) of the theorem statement.
For any $x, y$, if $h^\star_f(x) \ne f(x)$ then it follows that $h^\star(x) \ne y$.
\end{proof}

% \subsubsection{A Separation in Sample Complexity}

% \begin{theorem}
% There exists a hypothesis class \Hyp that has uniform convergence with complexity $m_\Hyp^\text{UC}(\epsilon, \delta)$, but with probability at least $1 - \delta$, samples of size $m^\text{G}(\epsilon, \delta) \ll m^\text{UC}(\epsilon, \delta)$ from any distribution \D are $\epsilon$-sufficient for grounding.
% \end{theorem}
% \begin{proof}
% Compose conjunctive propositional formulas with general propositional formulas.
% The former has $m_\Hyp^{UC}(\epsilon, \delta) = n\log(\nicefrac{3}{\delta})/\epsilon$, whereas the latter has $m_\Hyp^{UC}(\epsilon, \delta) = 3^n\log(\nicefrac{3}{\delta})/\epsilon$.
% Combining them gives something like $m_\Hyp^{UC}(\epsilon, \delta) = 3^{n+1}\log(\nicefrac{3}{\delta})/\epsilon$.
% If the problem is decomposable so that $\phi$ corresponds to the general propositional formula, then we should be able to show that $m^\text{G}(\epsilon, \delta) = n\log(\nicefrac{3}{\delta})/\epsilon$, because we just need to do ERM on the conjunctive part of the data.
% \end{proof}

% \subsection{Non-Bijective Problems}

Without conditions like (1) from Theorem~\ref{lemma:bijective-learnable}, which essentially provide that solutions to $\phi$ behave like a bijective function, it is less clear when \ermphi will succeed.
The central issue is that if $\phi$ admits multiple compatible groundings for a given output $y$, then in order to solve \ermphi the learner will need to discern which grounding is correct in order to identify the correct hypothesis $h_f$.
Definition~\ref{def:groundable} relates a class of problems for which this uncertainty is resolved by two factors: a notion of regularity on the companion hypothesis class $\Hyp_f$ that limits the extent to which candidates can behave ``erratically'' on a given sample, and a property of the data which ensures that grounding consistency implies correctness with increasing probability in $|S|$.

\begin{definition}[Groundable Problem]
\label{def:groundable}
Let \D, \Hyp be decomposable by first-order theory \T with constants in \Z, grounding function $f$ and prediction logic $\phi$.
Then \D, \Hyp is \emph{groundable} with monotonically increasing rate $\delta : \mathbb{N} \to [0,1]$ if for any $n > 0$:
\begin{enumerate}
	\item For any $S \sim \D^n$, there exists a hypothesis $h_f \in \Hyp_f$ that is consistent with all of $S$, i.e. for all $(x, y) \in S$, $\phi(h_f(x), y)$ is true.
	\item For all grounding hypotheses $h_f$ in the companion hypothesis space $\Hyp_f$, 
	\[
		\Pr_{S \sim \D^n}\left[
			\forall (x, y) \in S. \phi(h_f(x), y) \Longrightarrow h_f(x) = f(x)
		\right]
		\ge \delta(n)
	\]
	In words, with probability increasing in the size of a sample $S$, whenever $h_f$ is consistent with the prediction logic over all of $S$ then it also matches the true grounding function $f$.
\end{enumerate}
\end{definition}

\begin{remark}
A class of problems that we conjecture might often meet the requirements of Definition~\ref{def:groundable} are those with distributions satisfying isoperimetric inequalities like the notion of $c$-isoperimetry given in~\cite{bubeck21robustness}, or mixtures thereof, and hypothesis classes of Lipschitz functions.
These conditions imply that grounding hypotheses will be nearly subgaussian on the data, satisfying measure concentration properties conducive to establishing the rate $\delta(n)$ needed in the second condition of Definition~\ref{def:groundable}.
\end{remark}

\begin{example}[Groundability of visual algebra]
\label{ex:visual-alg-groundable}
The visual algebra problem from Example~\ref{ex:visual-alg} is groundable for certain hypothesis classes.
To understand why intuitively, we start by making the assumption that all grounding hypotheses $h_f$ consistently map the numbers in an instance to the same bitvector constant.
In other words, $h_f$ will map any appearance of ``4'' to the same bitvector, although it may not be the correct one, e.g., it will not map a four to $\mathsf{0001}$ in one instance and $\mathsf{0100}$ in another.
This ensures that (2) from Definition~\ref{def:groundable} will hold.

Suppose that we are given a sample containing the instances $3x + 5 = 11$, $7x + 3 = 10$, $\ldots$, and at least eight others.
Then the set of hypotheses that could be consistent with $\phi$ on both instances are those satisfying a linear system that corresponds to the arithmetic in $\phi$:
\[
\begin{array}{ccc}
2 \cdot h_f(3) + h_f(5) - 10 \cdot h_f(1) - h_f(1) & = & 0 \\
1 \cdot h_f(7) + h_f(3) - 10 \cdot h_f(1) - h_f(0) & = & 0 \\
\vdots & & 
\end{array}
\]
With high probability, this system has a unique solution.

The assumption that $h_f$ will consistently map different visual representations of digits to the same bitvectors is too simplistic for realistic hypothesis classes, but may hold with high probability assuming the hypothesis class contains at least one member that is consistent on the sample.
If the sample is sufficiently large and $h_f$ does not map digits consistently, then it is very unlikely that it will also be consistent with $\phi$ universally across the sample, so the event inside the probability in Definition~\ref{def:groundable} is vacuously true.
The only hypotheses for which the antecedent has a reasonable chance of being true are those that consistently map instances to bitvectors, which by the reasoning given above, are almost certain to be the true grounding function $f$.
$\square$
\end{example}

We conclude this section with Theorem~\ref{thm:groundable}, which shows that problems satisfying Definition~\ref{def:groundable} have good \ermphi solutions with probability strictly increasing in sample size.

\begin{theorem}[Groundable $\rightarrow$ learnable]
\label{thm:groundable}
Let \D, \Hyp be a \T-decomposable problem, for decidable theory \T, that satisfies the following properties.
\begin{enumerate}
	\item \D, \Hyp is groundable with rate $\delta_1$.
	% \item For any sample $S \sim \D^n$, there exists a hypothesis $h_f \in \Hyp_f$ that is consistent with all of $S$, i.e. for all $(x, y) \in S$, $\phi(h_f(x), y)$ is true.
	\item There exists a decreasing function $\delta_2 : \mathbb{N} \to [0, 1]$ such that samples $S \sim \D^n$ fail to be $\nicefrac{\epsilon}{2}$-sufficient for grounding with $L^{01}$ with probability at most $\delta_2(n)$.
	\item For any $(x, y)$ in the support of \D, $|\{z : \phi(z, y)\}|$ is finite.
\end{enumerate}
Then the \ermphi solution $\hat{h}$ yields:
\[
	\Pr_{S \sim \D^n}[
		L^{01}_\D(\hat{h}) \le \min_{h \in \Hyp}\,L^{01}_\D(h) + \epsilon
	] 
	\ge \delta_1(n) \cdot (1 - \delta_2(n))
\]
\end{theorem}
\begin{proof}
The argument for this result follows much of the same reasoning as used in the proof of Lemma~\ref{lemma:bijective-learnable}, with one major exception.
We construct an algorithm that uses a \T-solver to generate a grounding sample for which it can derive an empirical minimizer from the companion hypothesis space, and return $\lambda x.g(\langle x \rangle_{h_f,\phi})$ as the final hypothesis.

However, $\phi$ may have more than one compatible grounding term for each output.
The algorithm generates all of them, denoted by the set $\mathcal{S}_f$.
\begin{equation}
\mathcal{S}_f = \{S_f : \forall 0 \le i < n. \exists x, y, z. \phi(z, y) \land S[i] = (x, y) \land S_f[i] = (x, z) \}
\end{equation}
Constructing $\mathcal{S}_f$ is possible in light of assumption (3) from the theorem statement. 
Let $h^\star$ be the model obtained by minimizing empirical risk over the potential samples in $\mathcal{S}_f$, i.e.,
\begin{equation}
\label{eq:hstar_def}
\hat{h}_f = \argmin_{h_f \in \Hyp_f} L^{01}_S (\lambda x.g(\langle x \rangle_{h_f},\phi)),
\quad\quad
\hat{h} = \lambda x.g(\langle x \rangle_{\hat{h}_f},\phi)
\end{equation}
Let $\hat{S}_{f}$ be the sample chosen to minimize Equation~\ref{eq:hstar_def}.
With probability at least $\delta_1(n)$, this is the correct grounding sample for $S$.
This follows by Definition~\ref{def:groundable}, which says that with probability no less than $\delta_1(n)$, $\hat{h}_{f}$ coincides with $f$ throughout $S$ whenever it is consistent with $\phi$ everywhere, i.e., whenever  $\phi(h_f(x), y)$ for all $(x, y) \in S$.
We know that $\hat{h}_f$ minimizes empirical risk on $S$, and that there is always a hypothesis that is consistent with $\phi$ everywhere on $S$ (Definition~\ref{def:groundable}), so this condition must hold.

Now assume that $S$ is $\nicefrac{\epsilon}{2}$-sufficient for grounding. 
Then we have that $L^{01}_{\D_f}(\hat{h}_f) \le L^{01}_{\hat{S}_{f}}(\hat{h}_f)  + \nicefrac{\epsilon}{2}$.
By reasoning identical to that used to prove Lemma~\ref{lemma:bijective-learnable}, we can obtain that
\begin{equation}
\label{eq:groundable_learnable_final}
L^{01}_\D(\hat{h}) \le \min_{h \in \Hyp}\,L^{01}_\D(h) + \epsilon
\end{equation}
The theorem states that $S$ is $\nicefrac{\epsilon}{2}$-sufficient for grounding with probability at least $1 - \delta_2(n)$.
In the worst case, this event is independent of whether $\hat{h}_f$ is consistent with $f$ everywhere on $S$, so Equation~\ref{eq:groundable_learnable_final} will be true with probability at least $\delta_1(n) \cdot (1 - \delta_2(n))$.
\end{proof}

We end this section with a remark about the likely separation in sample complexity for MNIST addition.
While it is not possible to prove such a claim without making fairly strong assumptions about the empirical MNIST dataset, our results in Section~\ref{sect:eval} provide evidence to suggest that this separation exists.

\begin{remark}
Recall from Example~\ref{ex:grounding-addition-algebra} that for an appropriate hypothesis class, a sufficient sample for MNIST addition need only contain $\nicefrac{1}{10}$ of the examples needed to adequately specify the task of addition, i.e., roughly that many fewer examples than would be needed to learn via ERM.
If the problem were instead ``$n$-bit'' MNIST addition, over pairs of images of digits $0, \ldots, 2^{n}-1$ then we might extrapolate that a sufficient \ermphi sample would still only require on the order of $2^n$ examples, whereas ERM would require on the order of $4^n$ additional examples, as it would still need to see all of the $(2^n-1)^2$ pairs to correctly learn the addition component of the task.
Example~\ref{ex:visual-alg-groundable} reasoned about the likelihood with which visual algebra satisfies Definition~\ref{def:groundable}, and we might apply similar reasoning to conjecture that MNIST addition does also.
Then Theorem~\ref{thm:groundable} implies a separation in sample complexity between the ERM and \ermphi variants of this problem.
We believe that this is illustrative of the promise brought by leveraging symbolic knowledge in learning.
\end{remark}
